Pruned Pivot: Correlation Clustering Algorithm for Dynamic, Parallel, and Local Computation Models

Given a graph with positive and negative edge labels, the correlation clustering problem aims to cluster the nodes so to minimize the total number of between-cluster positive and within-cluster negative edges. This problem has many applications in data mining, particularly in unsupervised learning. Inspired by the prevalence of large graphs and constantly changing data in modern applications, we study correlation clustering in dynamic, parallel (MPC), and local computation (LCA) settings. We design an approach that improves state-of-the-art runtime complexities in all these settings. In particular, we provide the first fully dynamic algorithm that runs in an expected amortized constant time, without any dependence on the graph size. Moreover, our algorithm essentially matches the approximation guarantee of the celebrated Pivot algorithm.

==> header/packages-arxiv.tex <==
\usepackage[utf8]{inputenc}
%% full size page
\usepackage{fullpage}
% \usepackage[margin = 2.5cm]{geometry}

% %% AMS packages
\usepackage{amsmath, amssymb, amsthm}

% %% graphics and colors
\usepackage{graphicx}
\usepackage{color}
\usepackage[usenames,dvipsnames]{xcolor}

\usepackage{tikz-qtree}  
\usepackage{tcolorbox}
%%bibliography
\usepackage{natbib}
\definecolor{Blue}{HTML}{2D2F92}
\definecolor{BrickRed}{rgb}{0.8, 0.25, 0.33}

\usepackage[hyperindex,breaklinks]{hyperref}
\hypersetup{
    colorlinks = true,
    linkcolor = black,
    citecolor = Blue,
    urlcolor = black
}

%%misc
\usepackage{nicefrac}


% \usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}



% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

\RequirePackage{algorithm}
\RequirePackage{algorithmic}



% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{xspace}




% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}



==> paper/intro.tex <==
\section{Introduction}
We study algorithms for the Correlation Clustering problem, which has many applications in Machine Learning and Data Mining~\cite{bansal2004correlation,becker2005survey,kalashnikov2008web,arasu2009large,firman2013learning,bonchi2013overlapping,li2017motif}.
Among the most prominent applications is clustering products into categories or detecting communities based on product co-purchasing~\cite{wang2013scalable,veldt2020parameterized,shi2021scalable}.
In this problem, we are given a set of objects with ``similar" or ``dissimilar" labels between every pair of objects, and the goal is to cluster these objects such that similar objects are in the same cluster and dissimilar objects are in different clusters. Formally, given a complete graph with edge weights in $\mathbb{R}$, correlation clustering with the \emph{minimum disagreement} objective asks to cluster the nodes such that the sum of the weights of positive edges between clusters plus the sum of the weights of negative edges inside clusters is minimized.\footnote{Correlation clustering has also been studied on weighted graphs and with other objectives such as \emph{maximum agreement} or \emph{minimum $\ell_p$ norm}
\cite{bansal2004correlation,swamy2004correlation,charikar2005clustering,demaine2006correlation,puleo2016correlation,
charikar2017local,ahmadi2019min,jafarov2021local,kalhan2019correlation}.} This paper focuses on the unweighted setting, where weights are in $\{-1,+1\}$. 

Correlation Clustering is APX hard~\cite{charikar2005clustering}. There has been a long line of work on approximation algorithms for correlation clustering; see e.g., \citet{bansal2004correlation,charikar2005clustering,demaine2006correlation,chawla2015near,jafarov2021local,cohen2022correlation,BCMT,chakrabarty2023single,cohen2023handling}.
The best known approximation factor is $1.437$ due to \citet*{cao2024understanding}.\footnote{The proof of $1.437$ approximation is computer-assisted, but the same publication also presents an analytical proof of $1.49$ approximation.} However, all known algorithms with approximation factors less than $3$ use linear programming (LP), which makes most of them impractical for dealing with massive data. 

In their seminal work, \citet*{pivot} introduced an elegant $3$-approximation algorithm called \Pivot, which runs in linear time (time proportional to the number of positive \emph{edges} in the graph). It is the algorithm of choice in practice. The algorithm has been adapted for various computational models including semi-streaming \cite{behnezhad2023single,cambus2022parallel,chakrabarty2023single}, parallel algorithms (MPC)~\cite{cambus2022parallel,BCMT}, local computation algorithms (LCA) \cite{BCMT}, and dynamic algorithms (\citet{BCMT}; see also \citet{chechik2019fully}).


We study correlation clustering for massive and dynamic graphs. Such graphs are used to represent 
social networks~\cite{tantipathananandh2011finding,hafiene2020influential}, knowledge graphs~\cite{fang2020dynamic,yan2021dynamic}, and user-product interactions~\cite{ding2019user}.
We design a \pivot-like algorithm that can be easily implemented in the fully dynamic regime and LCA and MPC models. Our algorithm is inspired by the recent works by \citet*{BCMT} and 
\citet*{chakrabarty2023single}.
\citet{BCMT} presented a $(3+\eps)$-approximate algorithm, called $R$-pivot, that runs in $O(\frac{1}{\eps})$ MPC rounds, for any $\eps>0$. 
This algorithm can be implemented in LCA with $\Delta^{O(1/\eps)}$-probe complexity, where $\Delta$ is the maximum node degree in the graph (consisting of positive edges). \citet{chakrabarty2023single} give a $(3+\eps)$-approximate semi-streaming algorithm that uses $O(n/\varepsilon)$ words of memory.
\citet{behnezhad2019fully} show how to maintain the lexicographically first maximal matching in a fully dynamic graph. Their result can be used to implement \Pivot in the fully dynamic setting. The expected update time for relabelling edges is $O(\log^2{n}\log^2{\Delta})$ per operation. \citet{chechik2019fully} provide a similar result for maximal matching with expected worst-case running time $O(\log^4{n})$ per update.


\subsection{Our Contributions}
In this paper, we provide a new variant of \Pivot, which we call \ourPivot, that gives a $(3+\eps)$-approximation for Correlation Clustering (see Theorem~\ref{thm:approx-factor}).
Our algorithm is local and parallelizable by design: Given a node $u$ and common randomness, it returns the cluster of $u$ after exploring only $O(1/\eps)$ nodes of the entire graph. 
This makes it easy to implement \ourPivot in various computational models, including dynamic algorithms, MPC, and LCA.

Our first result is an efficient algorithm for dynamically maintaining a clustering. This is the first dynamic algorithm for Correlation Clustering, whose expected running time does not depend on the graph size. 

\begin{theorem}[Fully-dynamic correlation clustering]\label{cor:dynamic}
For any $\eps>0$, there is a data structure that maintains a $3+\eps$ approximation of correlation clustering in a fully-dynamic setting with an oblivious adversary. The expected update time is $O(1/\eps)$ per operation. 
\end{theorem}
\cref{cor:dynamic} gives an almost $3$ approximation fully dynamic algorithm with update time $O(1)$, which answers an open question posed by \citet{BCMT}.

\begin{theorem}[Correlation clustering in MPC]\label{cor:MPC}
    For any $\eps>0$, there is a randomized $O(\log{\frac{1}{\eps}})$-round MPC algorithm that achieves a $3+\eps$ approximation for Correlation Clustering. This bound holds even when each machine has a memory sublinear in the node-set size.
\end{theorem}
The previously best-known MPC algorithm by \citet{BCMT} requires $O(1/\eps)$ rounds. Hence, our approach improves the dependence on $1/\eps$ exponentially.
\begin{theorem}[Correlation clustering in LCA]\label{cor:LCA}
For any $\eps>0$, there is a randomized $O(\Delta / \eps)$-probe complexity local computation algorithm that achieves a $3+\eps$ approximation of correlation clustering on graphs with maximum 
degree~$\Delta$.
\end{theorem}
\cref{cor:LCA} gives an almost $3$ approximation LCA in, essentially, $O(\Delta)$ probes, thus answering another question posed by \citet*{BCMT}. 
The previously best-known algorithms for LCA were the algorithm by \citet{BCMT} giving $3+\eps$ approximation in $\Delta^{O(1/\eps)}$ probes, and
the work by \citet{behnezhad2023single} providing a $5$-approximate algorithm in $O(\poly \log n)$ space and $O(\Delta \cdot \poly \log n)$ probes.\footnote{Our LCA algorithm uses $O(\Delta / \eps \cdot \poly \log n)$ space.}


We provide empirical evaluations on synthetic graphs in \cref{sec:empirical}. They show that exploring only $4$ nodes to obtain a node's clustering suffices for the cost of \ourPivot to be within $1\%$ of the cost of \pivot.

Moreover, in \cref{section:pram} we describe how to implement our algorithm in the CRCW PRAM model in $O(1/\eps)$ rounds.

We finally note that our main technical result (\cref{thm:bound-X-Q}) is of independent interest.
A seminal work by \citet*{yoshida2009improved} shows how to learn whether a randomly chosen node is in MIS using the average-degree LCA probes.
Our work essentially recovers that claim using a significantly different analysis.



\subsection{Comparison to prior work}
Several closely related works have introduced variants of the \pivot algorithm. In \pivot, nodes are processed according to a predefined and random order, and each node queries its neighbors that have already been processed to determine its cluster (for a formal description of \Pivot see \cref{sec:pivot}). Hence, to determine the cluster of each node, multiple   ``query paths" are made, and the collection of these query paths makes a ``query tree". (For a more formal definition of query paths and query trees, refer to \cref{sec:querypaths}.)

First, given a parameter $R$, the $R$-\pivot algorithm by \citet{BCMT} runs the \pivot algorithm but only considers ``query paths" of depth at most $R$. If, to obtain the cluster of a node, one needs to consider query paths of length more than $R$, then this node is put into a singleton cluster. \citet{BCMT} show that this algorithm has approximation factor $3+O(\frac{1}{R})$.

Second, the semi-streaming algorithm by~\citet{chakrabarty2023single} is another modified version of \pivot. In this approach, given a parameter $R$, every node only queries at most its $R$ top-ranked neighbors when deciding on their cluster. This algorithm yields an approximation factor of $3 + O(\frac{1}{R})$. 
%We call this algorithm Narrow-\Pivot.

In \ourPivot, instead of only limiting the number of neighbors each node queries or the depth of the query paths, our algorithm limits \emph{the total size} of the query tree. Our analysis of the algorithm uses a new approach to counting query and \emph{expensive} paths, which is very different from the approach of \citet{BCMT}.



Our main technical contribution is a proof that by limiting the total size of the query tree, the existence/non-existence of each edge only influences at most a constant number of other nodes. This crucial point allows us to achieve low probe complexity in LCA and MPC, and constant update time in the dynamic setting. %\mina{mention empirical evaluation}





